Moving on from OntoNotes: Coreference Resolution Model Transfer

Academic neural models for coreference resolution (coref) are typically trained on a single dataset, OntoNotes, and model improvements are benchmarked on that same dataset. However, real-world applications of coref depend on the annotation guidelines and the domain of the target dataset, which often differ from those of OntoNotes. We aim to quantify transferability of coref models based on the number of annotated documents available in the target dataset. We examine eleven target datasets and find that continued training is consistently effective and especially beneficial when there are few target documents. We establish new benchmarks across several datasets, including state-of-the-art results on PreCo.

==> Moving on from OntoNotes Coreference Resolution Model Transfer (EMNLP arxiv final)_arXiv/benchmark.tex <==
\begin{table*}
    \centering
    \setlength{\tabcolsep}{3pt}
    \small
    \begin{tabular}{cccccc}
    \toprule
    Dataset & Prior work & Previous Model & Previous Score & Our best & Our Model \\
    \midrule
     PreCo  & \citet{wu2020understanding}  & SpanBERT + C2F & 85.0 & {\bf 88.0} & \textsc{pc}\\
     LitBank & \citet{thirukovalluru-etal-2021-scaling} & SpanBERT + C2F & {\bf 78.4} & 76.7 & \textsc{on} \\
     QBCoref & \citet{guha-etal-2015-removing} & Berkeley & $<35$ & {\bf 78.1} & \textsc{on} \\
     ARRAU\textsuperscript{RST} &  \citet{yu-etal-2020-cluster} & BERT + cluster ranking & 77.9 & {\bf 79.1}* & \textsc{pc} \\
     SARA & \newcite{holzenberger-etal-2021-factoring} & string match baselines & 55.1 & {\bf 72.9} & \textsc{on} \\
     \midrule
     OntoNotes\textsuperscript{zh}  & \citet{chen-ng-2012-chinese} & Multi-pass sieve & 62.2 & {\bf 69.0} & \textsc{en}\\
     OntoNotes\textsuperscript{ar}  & \citet{aloraini-etal-2020-neural} & AraBERT + C2F & {\bf 63.9} & 58.5 & \textsc{en}\\
     SemEval\textsuperscript{ca}  & \citet{attardi-etal-2010-tanl} & feature-based + MaxEnt & 48.2 &  {\bf 51.0} & \textsc{en}\\
     SemEval\textsuperscript{es}  & \citet{attardi-etal-2010-tanl} & feature-based + MaxEnt & 49.0 &  {\bf 51.3} & \textsc{en}\\
     SemEval\textsuperscript{it}  &  \citet{kobdani-schutze-2010-sucre} & feature-based + decision tree & {\bf 60.8} & 36.7 & \textsc{en}\\
     SemEval\textsuperscript{nl}  & \citet{kobdani-schutze-2010-sucre} & feature-based + decision tree & 19.1  & {\bf 55.4} & \textsc{en}\\
    \bottomrule
    \end{tabular}
    \caption{Test F\textsubscript{1} on all datasets and the previous state-of-the-art on each dataset, to the best of our knowledge. Again, we are benchmarking the general method of continued training described in this paper, which will not necessarily outperform models that incorporate domain or language specific knowledge. Our best \textsc{Transfer} model is determined by the dev set (\autoref{sec:appendix:training}). *ARRAU\textsuperscript{RST} is not directly comparable to prior work as we test on a slightly differently-preprocessed subset. Multi-pass sieve \cite{raghunathan-etal-2010-multi}, Berkeley \cite{durrett-klein-2013-easy}, and C2F \cite{lee-etal-2018-higher} refer to widely-used coreference resolution models.}
    \label{tab:data:benchmark}
    \setlength{\tabcolsep}{6pt}
\end{table*}


==> Moving on from OntoNotes Coreference Resolution Model Transfer (EMNLP arxiv final)_arXiv/dataset_stats.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{crrrr}
    \toprule
     Dataset & Training & Dev & Test & \# Folds \\
    \midrule
     OntoNotes\textsuperscript{en} & 2,802 & 343 & 348 & - \\
     OntoNotes\textsuperscript{zh} & 1,810 & 252 & 218 & - \\
     OntoNotes\textsuperscript{ar} & 359 & 44 & 44 & - \\
     PreCo & 36,120 & 500 & 500 & - \\
     LitBank & 80 & 10 & 10 & 10 \\
     QBCoref & 240 & 80 & 80 & 5 \\
     ARRAU\textsuperscript{RST} & 335 & 18 & 60 & - \\
     SARA & 138 & 28 & 28 & 7 \\
     Semeval\textsuperscript{ca} & 829 & 142 & 167 & - \\
     Semeval\textsuperscript{es} & 875 & 140 & 168 & - \\
     Semeval\textsuperscript{it} & 80 & 17 & 46 & - \\
     Semeval\textsuperscript{nl} & 145 & 23 & 72 & - \\
    \bottomrule
    \end{tabular}
    \caption{Number of documents for each of the datasets considered in this work. For the smaller datasets, we perform $k$-fold cross-validation. }
    \label{tab:data:stats}
\end{table}


==> Moving on from OntoNotes Coreference Resolution Model Transfer (EMNLP arxiv final)_arXiv/figure1.5.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{rq5_f1_small.pdf}
    \caption{Like \autoref{fig:rq1links}, this plot demonstates the effectiveness of continued training across different \textit{languages}. \textsc{XLM-R} uses a pretrained encoder (dashed line), while \textsc{Transfer (en)} is first trained on OntoNotes\textsuperscript{en} (solid line). Trends on mention accuracy and using gold mentions look similar and are in \autoref{sec:appendix:layers}.}
    \label{fig:rq5links}
\end{figure*}

==> Moving on from OntoNotes Coreference Resolution Model Transfer (EMNLP arxiv final)_arXiv/figure1.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{rq1_f1_big.pdf}
    \caption{Each subplot shows the test performance for each model and (English) dataset when trained with a different number of documents. The first and second rows are coreference and mention boundary F\textsubscript{1} in the end-to-end setting, while the third row is the coreference F\textsubscript{1} with gold mentions. \textsc{SpanBERT} is a pretrained encoder, while the \textsc{SpanBERT-On} encoders are further finetuned on OntoNotes by \citet{joshi-etal-2020-spanbert}, with \textbf{b}ase and \textbf{L}arge designating its size. Unlike these (dashed lines) models for which we initialize the encoder, the \textsc{Transfer} models (solid lines) use continued training and initialize the full model with one that has already been trained on a source dataset, either OntoNotes (on) or PreCo (pc).}
    \label{fig:rq1links}
\end{figure*}

==> Moving on from OntoNotes Coreference Resolution Model Transfer (EMNLP arxiv final)_arXiv/figure2.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{rq2_f1.pdf}
    \caption{The expected test F\textsubscript{1} (and standard deviation) on the PreCo dataset for a given number of training documents and 20 sampled subsets of dev documents for two models described in Section \ref{sec:data:source}. The number of runs matching the best full dev checkpoint is in the lower-right. We find that the dev set size has relatively little impact.}
    \label{fig:rq2dev}
\end{figure*}


==> Moving on from OntoNotes Coreference Resolution Model Transfer (EMNLP arxiv final)_arXiv/figure3.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{rq3_rq6_f1.pdf}
    \caption{Average F\textsubscript{1} of the models on both the target and the original datasets as different number of (target) training examples are used in continued training. The dashed lines are the scores on the target dataset (mirroring \autoref{fig:rq1links}) while the solid lines show performance on the original dataset.}
    \label{fig:rq3}
\end{figure*}


==> Moving on from OntoNotes Coreference Resolution Model Transfer (EMNLP arxiv final)_arXiv/figure4.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{rq4_f1.pdf}
    \caption{Average F\textsubscript{1} across different models and number of trainable layers. \textit{Low} vs. \textit{All} describes the number of documents used for the first fold of LitBank (10 vs. 80) and QBCoref (15 vs. 240).}
    \label{fig:rq4}
\end{figure}


==> Moving on from OntoNotes Coreference Resolution Model Transfer (EMNLP arxiv final)_arXiv/figure4_full.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.7\linewidth]{rq4_f1_large.pdf}
    \caption{Average F\textsubscript{1} across different models and number of trainable layers, varying between 0, 6, 12 or 24 layers. \textit{Low} vs. \textit{Medium} vs. \textit{All} describes the number of documents used for the first fold of LitBank (10, 40, 80 documents), QBCoref (15, 60, 240 documents), and OntoNotes\textsuperscript{zh} (50, 500, 1810 documents). The initialization methods follow those used throughout the paper.}
    \label{fig:rq4_full}
\end{figure*}


==> Moving on from OntoNotes Coreference Resolution Model Transfer (EMNLP arxiv final)_arXiv/figure5_large.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{rq5_f1_big.pdf}
    \caption{Full version of \autoref{fig:rq5links}. Like \autoref{fig:rq1links}, this plot demonstates the effectiveness of continued training across different \textit{languages}. \textsc{XLM-R} uses a pretrained encoder (dashed line), while \textsc{Transfer (en)} is first trained on OntoNotes\textsuperscript{en} (solid line).}
    \label{fig:rq5links_large}
\end{figure*}
